Deep learning for low-magnitude earthquake detection on a multi-level sensor network

Automatic detection of low-magnitude earthquakes has become an increasingly important research topic in recent years due to a sharp increase in induced seismicity around the globe. The detection of low-magnitude seismic events is essential for microseismic monitoring of hydraulic fracturing, carbon capture and storage, and geothermal operations for hazard detection and mitigation. Moreover, the detection of micro-earthquakes is crucial to understand the underlying mechanisms of larger earthquakes. Various algorithms, including deep learning methods, have been proposed over the years to detect such low-magnitude events. However, there is still a need for improving the robustness of these methods in discriminating between local sources of noise and weak seismic events. In this study, we propose a convolutional neural network (CNN) to detect seismic events from shallow borehole stations in Groningen, the Netherlands. We train a CNN model to detect low-magnitude earthquakes, harnessing the multi-level sensor configuration of the G-network in Groningen. Each G-network station contains four geophones at depths of 50, 100, 150, and 200 meters. Unlike prior deep learning approaches that use 3-component seismic records only at a single sensor level, we use records from the entire borehole as one training example. This allows us to train the CNN model using moveout patterns of the energy traveling across the borehole sensors to discriminate between events originating in the subsurface and local noise arriving from the surface. We compare the prediction accuracy of our trained CNN model to that of the STA/LTA and template matching algorithms on a two-month continuous record. We demonstrate that the CNN model shows significantly better performance than STA/LTA and template matching in detecting new events missing from the catalog and minimizing false detections.

==> Event detection using deep learning in Groningen/biography.tex <==
% !TEX root = main.tex
% Biographies
%
% If you have an EPS/PDF photo (graphicx package needed) extra braces are
% needed around the contents of the optional argument to biography to prevent
% the LaTeX parser from getting confused when it sees the complicated
% \includegraphics command within an optional argument. (You could create
% your own custom macro containing the \includegraphics command to make things
% simpler here.)
%\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{mshell}}]{Michael Shell}
% or if you just want to reserve a space for a photo:

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{../photo/denis.jpg}}]{Denis Anikiev} received the B.Sc. degreed in physics in 2008, the M.Sc. degree in geophysics in 2011 and the Ph.D. degree in geophysics in 2015 from St. Petersburg State University, St. Petersburg, Russian Federation.
  He is currently a scientist at the Helmholtz Centre Potsdam - GFZ German Research Centre for Geosciences, Potsdam, Germany, where he is also responsible for development of software tools for potential field modeling, coupled multi-physics finite-element modeling and machine learning.
  His research interests include various fields of geoscience: inverse problems, seismic imaging, seismology, wave phenomena in complex media, potential fields, data science and machine learning methods in geophysics.
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{../photo/umair.jpg}}]{Umair bin Waheed}
received the Ph.D. degree in Earth Science and Engineering from King Abdullah University of Science and Technology, Thuwal,
Saudi Arabia, in 2015. Currently, he is an Assistant Professor of Geophysics at the King Fahd University of Petroleum and Minerals (KFUPM). Prior to joining KFUPM, he was a post-doctoral fellow at the Department of Geosciences and a Fellow of Writing in Science and
Engineering at the Princeton Writing Program,
Princeton University. His research interests are broadly in the area of computational geosciences. Specifically, he is interested in automating and improving workflows through the use of smart algorithms for enhanced decision making in subsurface energy systems. 
\end{IEEEbiography}

\begin{IEEEbiography}{Naveed Iqbal}
Biography text here.
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{../photo/frantisek.jpg}}]{Franti\v{s}ek Stan\v{e}k} received his B.Sc., M.Sc. degrees in applied geology and in 2018 his Ph.D. degree in geophysics from Charles University, Czech Republic.
He is currently a postdoctoral fellow at Colorado School of Mines, Golden, Colorado, USA, where he joined Reservoir Characterization Project at Department of Geophysics.
His research interests include integrated reservoir characterization, microseismic monitoring of hydraulic fracturing, induced seismicity monitoring, and fiber-optic sensing applications in the oil and gas industry.
\end{IEEEbiography}

\begin{IEEEbiography}{Dmitry Alexandrov}
Biography text here.
\end{IEEEbiography}

\begin{IEEEbiography}{Leo Eisner}
Biography text here.
\end{IEEEbiography}


% if you will not have a photo at all:
% \begin{IEEEbiographynophoto}{John Doe}
% Biography text here.
% \end{IEEEbiographynophoto}

% insert where needed to balance the two columns on the last page with
% biographies
%\newpage

% \begin{IEEEbiographynophoto}{Jane Doe}
% Biography text here.
% \end{IEEEbiographynophoto}

% You can push biographies down or up by placing
% a \vfill before or after them. The appropriate
% use of \vfill depends on what kind of text is
% on the last page and whether or not the columns
% are being equalized.

%\vfill

% Can be used to pull up biographies so that the bottom of the last one
% is flush with the other column.
%\enlargethispage{-5in}


==> biography.tex <==
% !TEX root = main.tex
% Biographies
%
% If you have an EPS/PDF photo (graphicx package needed) extra braces are
% needed around the contents of the optional argument to biography to prevent
% the LaTeX parser from getting confused when it sees the complicated
% \includegraphics command within an optional argument. (You could create
% your own custom macro containing the \includegraphics command to make things
% simpler here.)
%\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{mshell}}]{Michael Shell}
% or if you just want to reserve a space for a photo:

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{../photo/denis.jpg}}]{Denis Anikiev} received the B.Sc. degreed in physics in 2008, the M.Sc. degree in geophysics in 2011 and the Ph.D. degree in geophysics in 2015 from St. Petersburg State University, St. Petersburg, Russian Federation.
  He is currently a scientist at the Helmholtz Centre Potsdam - GFZ German Research Centre for Geosciences, Potsdam, Germany, where he is also responsible for development of software tools for potential field modeling, coupled multi-physics finite-element modeling and machine learning.
  His research interests include various fields of geoscience: inverse problems, seismic imaging, seismology, wave phenomena in complex media, potential fields, data science and machine learning methods in geophysics.
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{../photo/umair.jpg}}]{Umair bin Waheed}
received the Ph.D. degree in Earth Science and Engineering from King Abdullah University of Science and Technology, Thuwal,
Saudi Arabia, in 2015. Currently, he is an Assistant Professor of Geophysics at the King Fahd University of Petroleum and Minerals (KFUPM). Prior to joining KFUPM, he was a post-doctoral fellow at the Department of Geosciences and a Fellow of Writing in Science and
Engineering at the Princeton Writing Program,
Princeton University. His research interests are broadly in the area of computational geosciences. Specifically, he is interested in automating and improving workflows through the use of smart algorithms for enhanced decision making in subsurface energy systems. 
\end{IEEEbiography}

\begin{IEEEbiography}{Naveed Iqbal}
Biography text here.
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{../photo/frantisek.jpg}}]{Franti\v{s}ek Stan\v{e}k} received his B.Sc., M.Sc. degrees in applied geology and in 2018 his Ph.D. degree in geophysics from Charles University, Czech Republic.
He is currently a postdoctoral fellow at Colorado School of Mines, Golden, Colorado, USA, where he joined Reservoir Characterization Project at Department of Geophysics.
His research interests include integrated reservoir characterization, microseismic monitoring of hydraulic fracturing, induced seismicity monitoring, and fiber-optic sensing applications in the oil and gas industry.
\end{IEEEbiography}

\begin{IEEEbiography}{Dmitry Alexandrov}
Biography text here.
\end{IEEEbiography}

\begin{IEEEbiography}{Leo Eisner}
Biography text here.
\end{IEEEbiography}


% if you will not have a photo at all:
% \begin{IEEEbiographynophoto}{John Doe}
% Biography text here.
% \end{IEEEbiographynophoto}

% insert where needed to balance the two columns on the last page with
% biographies
%\newpage

% \begin{IEEEbiographynophoto}{Jane Doe}
% Biography text here.
% \end{IEEEbiographynophoto}

% You can push biographies down or up by placing
% a \vfill before or after them. The appropriate
% use of \vfill depends on what kind of text is
% on the last page and whether or not the columns
% are being equalized.

%\vfill

% Can be used to pull up biographies so that the bottom of the last one
% is flush with the other column.
%\enlargethispage{-5in}

